Multimodal Abstractive Summarization of Instructional Videos with Vision-Language Models

Multimodal video summarization requires visual features that align semantically with language generation. Traditional approaches rely on CNN features trained for object classification, which represent visual concepts as discrete categories not aligned with natural language. We propose ClipSum, a framework that leverages frozen CLIP vision-language features with explicit temporal modeling and dimension-adaptive fusion for instructional video summarization. CLIP's contrastive pre-training on 400M image-text pairs yields visual features semantically aligned with the linguistic concepts that text decoders generate, bridging the vision-language gap at the representation level. On YouCook2, ClipSum achieves 33.0% ROUGE-1 versus 30.5% for ResNet-152 with 4x lower dimensionality (512 vs. 2048), demonstrating that semantic alignment matters more than feature capacity. Frozen CLIP (33.0%) surpasses fine-tuned CLIP (32.3%), showing that preserving pre-trained alignment is more valuable than task-specific adaptation. https://github.com/aqeeelmirza/clipsum

==> architecture_figure.tex <==
% Architecture Figure - Add to your LaTeX document
% Requires: 
\usepackage{tikz}
% Add after 
\usepackage declarations: \usetikzlibrary{shapes,arrows,positioning,calc}

\begin{figure*}[t]
\centering
\begin{tikzpicture}[
    node distance=1cm and 1.5cm,
    block/.style={rectangle, draw, fill=blue!20, text width=3cm, text centered, rounded corners, minimum height=1cm},
    smallblock/.style={rectangle, draw, fill=green!20, text width=2.5cm, text centered, rounded corners, minimum height=0.8cm},
    videoblock/.style={rectangle, draw, fill=orange!20, text width=2.5cm, text centered, rounded corners, minimum height=0.8cm},
    fusionblock/.style={rectangle, draw, fill=red!20, text width=3.5cm, text centered, rounded corners, minimum height=1cm},
    input/.style={rectangle, draw=none, text width=2.5cm, text centered},
    arrow/.style={thick,->,>=stealth}
]

% Video Path (Left)
\node[input] (video) {Video Frames\\(50 frames)};
\node[videoblock, below=of video] (clip) {CLIP ViT-B/32\\(Frozen)};
\node[smallblock, below=of clip] (temporal) {Temporal\\Encoding};
\node[videoblock, below=of temporal] (vtf) {Transformer\\Encoder};

% Text Path (Right)
\node[input, right=4cm of video] (text) {Procedural Text\\(Input)};
\node[smallblock, below=of text] (tokenizer) {BPE Tokenizer};
\node[block, below=of tokenizer] (embed) {Token\\Embedding};
\node[block, below=of embed] (encoder14) {BART Encoder\\Layers 1-4};

% Fusion Layer
\node[fusionblock, below=of encoder14] (fusion) {BART Encoder Layer 5\\+ Cross-Modal Attention};

% Final Encoder
\node[block, below=of fusion] (encoder6) {BART Encoder\\Layer 6};

% Decoder
\node[block, below=of encoder6] (decoder) {BART Decoder\\(6 layers)};

% Output
\node[input, below=of decoder] (output) {Generated\\Summary};

% Arrows - Video Path
\draw[arrow] (video) -- (clip);
\draw[arrow] (clip) -- node[right] {\small (50, 512)} (temporal);
\draw[arrow] (temporal) -- (vtf);

% Arrows - Text Path
\draw[arrow] (text) -- (tokenizer);
\draw[arrow] (tokenizer) -- (embed);
\draw[arrow] (embed) -- node[right] {\small (N, 768)} (encoder14);
\draw[arrow] (encoder14) -- (fusion);

% Fusion Arrow
\draw[arrow, red, thick] (vtf) -| ($(vtf)!0.5!(fusion)$) |- (fusion);

% Final Path
\draw[arrow] (fusion) -- (encoder6);
\draw[arrow] (encoder6) -- (decoder);
\draw[arrow] (decoder) -- (output);

% Labels
\node[left=0.3cm of clip, align=right, text=orange] {\textbf{Visual}\\Path};
\node[right=0.3cm of tokenizer, align=left, text=blue] {\textbf{Text}\\Path};
\node[right=0.3cm of fusion, align=left, text=red] {\textbf{Fusion}};

\end{tikzpicture}
\caption{Architecture overview of our multimodal abstractive summarization framework. Video frames are encoded through CLIP ViT-B/32 to obtain semantically-aligned visual features (512-dim), while procedural text is processed through BART encoder. Visual and textual representations are fused via cross-modal attention at encoder layer 5, and the decoder generates the abstractive summary.}
\label{fig:architecture}
\end{figure*}
